Search for new phenomena in events with at least three photons collected in $pp$ collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector

Results of a search for new phenomena in events with at least three photons are reported. Data from proton--proton collisions at a centre-of-mass energy of 8 TeV, corresponding to an integrated luminosity of 20.3 fb$^{-1}$, were collected with the ATLAS detector at the LHC. The observed data are well described by the Standard Model. Limits at the 95% confidence level on new phenomena are presented based on the rate of events in an inclusive signal region and a restricted signal region targeting the rare decay $Z\to 3\gamma$, as well as di-photon and tri-photon resonance searches. For a Standard Model Higgs boson decaying to four photons via a pair of intermediate pseudoscalar particles ($a$), limits are found to be $\sigma \times {\text {BR}}(h \rightarrow aa) \times {\text {BR}}(a \rightarrow \gamma \gamma)^{2} < 10^{-3} \sigma_{\text{SM}}$ for 10 GeV $< m_{a} <$ 62 GeV. Limits are also presented for Higgs boson-like scalars ($H$) for $m_{H} > $ 125 GeV, and for a $Z'$ decaying to three photons via $Z' \rightarrow a+\gamma \rightarrow 3\gamma$. Additionally, the observed limit on the branching ratio of the $Z$ boson decay to three photons is found to be BR$(Z \rightarrow 3\gamma) < 2.2 \times 10^{-6}$, a result five times stronger than the previous result from LEP.

==> MultiPhotonPaper_EventSamples.tex <==
The backgrounds from events with three or four hard process photons and electrons from Z decays are estimated with MC samples.  The ATLAS detector is fully simulated using {\sc Geant} 4~\cite{Agostinelli:2002hh}, and simulated events are reconstructed using the same software as that used for collision data.

The irreducible SM three or four photon backgrounds are modeled with {\sc MadGraph} 5.1.4.4~\cite{Alwall:2011uj} and {\sc Pythia} 8.163~\cite{Sjostrand:2007gs}, and two-photon processes are modeled with {\sc Pythia}.  Processes where a Z boson decays to an $e^{+}e^{-}$ pair, accompanied by a photon not from the matrix element, are modeled with {\sc Powheg-Box 1.0}~\cite{Alioli:2008tz}+{\sc Pythia}, and Z+$\gamma$ production is modeled with {\sc Sherpa} 1.4.1~\cite{Gleisberg:2008ta}.  Processes where a W boson decays to a lepton plus a neutrino in association with one or two hard-process photons and from 0 up to 2 jets are simulated with {\sc Alpgen}~\cite{Mangano:2002ea}+{\sc Herwig}~\cite{Corcella:2000bw,Corcella:2002jc}.

As an example of a BSM process to which this search is sensitive, simulated samples of a Higgs boson decaying into four photons via two intermediate pseudoscalar ({\it a}) particles are produced.  {\sc Powheg-Box} is used for the production of a Higgs via gluon-gluon fusion and {\sc Pythia8} for the decay of the Higgs into four photons, for the SM Higgs at $m_{h} = $ 125 GeV/c$^{2}$, for 30000 events for each of eleven $m_{a}$ points from 1 to 62 GeV/c$^{2}$, as well as twelve additional samples of 30000 events each for scalars and pseudoscalars with higher masses, four $m_{a}$ points each for $m_{h} = $ 300, 600, and 900 GeV/c$^{2}$.

Additionally, {\sc Pythia8} is used to produce simulated samples of processes arising in models~\cite{Toro:2012sv} that feature additional vector gauge bosons ($Z^{'}$) that can decay to a photon + {\it a}, with the subsequent decay of the {\it a} into a pair of photons, resulting in a three photon final state.  A total of 30000 events is generated and fully simulated for each of eighteen total mass points, three $m_{a}$ points each for $m_{Z^{'}} = $ 100, 200, 400, 600, 800 and 1000 GeV/c$^{2}$.

The rare process of a SM Z boson decaying into three photons is simulated with {\sc MadGraph5}, using a custom model produced with {\sc FeynRules}~\cite{Alloul:2013bka,Degrande:2011ua}, and using the calculated values of the dimensionful coupling constants expected from the appropriate SM Lagrangian terms, assuming the calculated SM branching ratio for this process.

The parton distribution functions for the {\sc MadGraph}, {\sc Pythia} and {\sc Alpgen + Herwig} samples are taken from CTEQ6L1~\cite{Pumplin:2002vw}; for the {\sc Powheg-Box} samples from CTEQ6M~\cite{Pumplin:2002vw}; and for the {\sc Sherpa} samples from CT10~\cite{PhysRevD.82.074024}.

Additionally, minimum bias pp interactions (pileup) in the same or nearby bunch crossings are modeled with {\sc Pythia}. All simulated events are re-weighted to reproduce the distribution of average number of interactions per bunch crossing ($\langle \mu \rangle$) observed in data over the course of the 2012 run.

==> MultiPhotonPaper_TitleAndAbstract.tex <==
Search for new phenomena in events with at least three photons collected in $pp$ collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector

Results of a search for new phenomena in events with at least three photons are reported.  Data from proton--proton collisions at a centre-of-mass energy of 8 TeV, corresponding to an integrated luminosity of 20.3 fb$^{-1}$, were collected with the ATLAS detector at the LHC.  The observed data are well described by the Standard Model.  Limits at the 95\% confidence level on new phenomena are presented based on the rate of events in an inclusive signal region and a restricted signal region targeting the rare decay $Z\to 3\gamma$, as well as di-photon and tri-photon resonance searches.  For a Standard Model Higgs boson decaying to four photons via a pair of intermediate pseudoscalar particles ($a$), limits are found to be $\sigma \times {\text {BR}}(h \rightarrow aa) \times {\text {BR}}(a \rightarrow \gamma \gamma)^{2} < 10^{-3} \sigma_{\text{SM}}$ for 10 GeV $< m_{a} <$ 62 GeV.  Limits are also presented for Higgs boson-like scalars ($H$) for $m_{H} > $ 125 GeV, and for a $Z'$ decaying to three photons via $Z' \rightarrow a+\gamma \rightarrow 3\gamma$.  Additionally, the observed limit on the branching ratio of the $Z$ boson decay to three photons is found to be BR$(Z \rightarrow 3\gamma) < 2.2 \times 10^{-6}$, a result five times stronger than the previous result from LEP.


==> Tables/ZprimeNCLimits.tex <==
     & 40 & 60 & 80 \\
 100 & 323.1 (395.0) & 152.3 (177.1) & 321.4 (381.9) \\
 \hline 
     & 50 & 100 & 150 \\
 200 & 80.8 (91.3) & 55.1 (63.5) & 53.1 (60.3) \\
 \hline 
     & 100 & 200 & 300 \\
 400 & 51.8 (64.2) & 45.0 (56.5) & 39.2 (47.8) \\
 \hline 
     & 100 & 250 & 400 \\
 600 & 40.9 (49.1) & 42.1 (52.6) & 42.1 (52.6) \\
 \hline 
     & 100 & 350 & 600 \\
 800 & 38.4 (47.9) & 35.5 (43.2) & 35.5 (43.2) \\
 \hline 
     & 100 & 450 & 800 \\
 1000 & 39.7 (47.2) & 54.4 (63.9) & 36.6 (43.2) \\
 \hline 

